Automated Detection of GDPR Disclosure Requirements in Privacy Policies using Deep Active Learning

Since GDPR came into force in May 2018, companies have worked on their data practices to comply with this privacy law. In particular, since the privacy policy is the essential communication channel for users to understand and control their privacy, many companies updated their privacy policies after GDPR was enforced. However, most privacy policies are verbose, full of jargon, and vaguely describe companies' data practices and users' rights. Therefore, it is unclear if they comply with GDPR. In this paper, we create a privacy policy dataset of 1,080 websites labeled with the 18 GDPR requirements and develop a Convolutional Neural Network (CNN) based model which can classify the privacy policies with an accuracy of 89.2%. We apply our model to perform a measurement on the compliance in the privacy policies. Our results show that even after GDPR went into effect, 97% of websites still fail to comply with at least one requirement of GDPR.

==> abstract.tex <==
Since GDPR came into force in May 2018, companies have worked on their data practices to comply with this privacy law. In particular, since the privacy policy is the essential communication channel for users to understand and control their privacy, many companies updated their privacy policies after GDPR was enforced. However, most privacy policies are verbose, full of jargon, and vaguely describe companies' data practices and users' rights. Therefore, it is unclear if they comply with GDPR. In this paper, we create a privacy policy dataset of 1,080 websites labeled with the 18 GDPR requirements and develop a Convolutional Neural Network (CNN) based model which can classify the privacy policies with an accuracy of 89.2\%. We apply our model to perform a measurement on the compliance in the privacy policies. Our results show that even after GDPR went into effect, 97\% of websites still fail to comply with at least one requirement of GDPR.
%Since the establishment of GDPR - a privacy law that has been heralded as the world's strongest protector of users' online privacy rights - hundreds of companies have changed their privacy policies to comply and avoid substantial fine. However, most privacy policies are verbose, full of jargon , and vaguely describe companies data practices and users' rights. Therefore, it is necessary to automate the compliance measurement of a privacy policy with privacy laws. In this paper, we describe a convolutional neural network based classification model that can classify the GDPR disclosure requirements in a privacy policy with an accuracy of 89.2\% and average F1-score as 0.88. We leveraged active learning technique to boost the performance of our classification model by 10.8\% while adding only 10.5\% additional training data. We created a privacy policy dataset containing 1080 online privacy policy documents labeled by experts with 18 GDPR requirements. We leveraged our classification model to measure the overall compliance  of  online privacy policies with GDPR and found six major GDPR requirements were implemented by only 4--15\% websites. Furthermore, we conducted a comprehensive user study to measure the effectiveness of the current privacy policy practices that are directly concerned with users' personal data and privacy rights, and report the results on 95 participants. Our overall study result shows that 25.8\% participants do not find the privacy policies relevant to GDPR to be helpful and 37\% participants think their privacy and rights over personal data, as disclosed in the privacy policy, may be violated by companies.
%ecessary to automate the compliance measurement of a privacy policy with privacy laws. In this paper, we describe a convolutional neural network based classification model that can classify the GDPR disclosure requirements in a privacy policy with an accuracy of 89.2\% and average F1-score as 0.88. We leveraged active learning technique to boost the performance of our classification model by 10.8\% while adding only 10.5\% additional training data. We created a privacy policy dataset containing 1080 online privacy policy documents labeled by experts with 18 GDPR requirements. We leveraged our classification model to measure the overall compliance  of  online privacy policies with GDPR and found six major GDPR requirements were implemented by only 4--15\% websites. Furthermore, we conducted a comprehensive user study to measure the effectiveness of the current privacy policy practices that are directly concerned with users' personal data and privacy rights, and report the results on 95 participants. Our overall study result shows that 25.8\% participants do not find the privacy policies relevant to GDPR to be helpful and 37\% participants think their privacy and rights over personal data, as disclosed in the privacy policy, may be violated by companies.
